Mesh Grading in Isogeometric Analysis

This paper is concerned with the construction of graded meshes for approximating so-called singular solutions of elliptic boundary value problems by means of multipatch discontinuous Galerkin Isogeometric Analysis schemes. Such solutions appear, for instance, in domains with re-entrant corners on the boundary of the computational domain, in problems with changing boundary conditions, in interface problems, or in problems with singular source terms. Making use of the analytic behavior of the solution, we construct the graded meshes in the neighborhoods of such singular points following a multipatch approach. We prove that appropriately graded meshes lead to the same convergence rates as in the case of smooth solutions with approximately the same number of degrees of freedom. Representative numerical examples are studied in order to confirm the theoretical convergence rates and to demonstrate the efficiency of the mesh grading technology in Isogeometric Analysis.

==> makefile <==
# enter your file name here
FILE = "MeshGrading"

# add any files that you might want tar to include
TAR_FILES = fig

# folder containing all files
FOLDER = notes


# set the page type
#PAGE_TYPE = letter
PAGE_TYPE = a4


######################################################################
####### DO NOT TOUCH ANYTHING BELOW THIS LINE ########################
######################################################################

# Executables

LATEX  = latex
BIBTEX = bibtex
DVIPS  = dvips
PS2PDF = ps2pdf
TAR    = tar
PDFLATEX = pdflatex

# Options

PS2PDF_FLAGS = -dPDFSETTINGS=/printer -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 -dUseCIEColor=true -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE="$(PAGE_TYPE)"
DVIPS_FLAGS  = -Ppdf -Pdownload35 -t $(PAGE_TYPE)

# Make

default: pdflatex

all:  bib pdf

pdflatex:
	$(PDFLATEX) $(FILE)

dvi:	
	$(LATEX) $(FILE)
	$(LATEX) $(FILE)

ps:	dvi
	$(DVIPS) $(DVIPS_FLAGS) -o $(FILE).ps $(FILE).dvi

pdf:	ps
	$(PS2PDF) $(PS2PDF_FLAGS) $(FILE).ps

bib:	dvi
	$(BIBTEX) $(FILE)
	$(LATEX) $(FILE)	
	$(LATEX) $(FILE)	

# Clean

clean:  
	\rm -rf auto *.blg *.aux *.dvi *.log *~ *.out

cleanall: clean tarclean
	\rm -rf ${FILE}.pdf ${FILE}.ps *.bbl

# Tarballs

tar:    
	$(TAR) cvfz $(FILE).tgz $(FILE).tex *.bib makefile $(TAR_FILES) --exclude .svn

tarall: clean
	cd ..; $(TAR) cvfz $(FILE)-all.tgz $(FOLDER) --exclude .svn --exclude *.tgz

submit: 
	$(TAR) cvfz $(FILE)-submit.tgz *.tex $(FILE).ps $(FILE).pdf \
		$(TAR_FILES) --exclude .svn --exclude *.tgz

tarclean:
	\rm -f $(FILE).tgz $(FILE)-submit.tgz ../$(FILE)-all.tgz

